Log2NS: Enhancing Deep Learning Based Analysis of Logs With Formal to Prevent Survivorship Bias

Analysis of large observational data sets generated by a reactive system is a common challenge in debugging system failures and determining their root cause. One of the major problems is that these observational data suffer from survivorship bias. Examples include analyzing traffic logs from networks, and simulation logs from circuit design. In such applications, users want to detect non-spurious correlations from observational data and obtain actionable insights about them. In this paper, we introduce log to Neuro-symbolic (Log2NS), a framework that combines probabilistic analysis from machine learning (ML) techniques on observational data with certainties derived from symbolic reasoning on an underlying formal model. We apply the proposed framework to network traffic debugging by employing the following steps. To detect patterns in network logs, we first generate global embedding vector representations of entities such as IP addresses, ports, and applications. Next, we represent large log flow entries as clusters that make it easier for the user to visualize and detect interesting scenarios that will be further analyzed. To generalize these patterns, Log2NS provides an ability to query from static logs and correlation engines for positive instances, as well as formal reasoning for negative and unseen instances. By combining the strengths of deep learning and symbolic methods, Log2NS provides a very powerful reasoning and debugging tool for log-based data. Empirical evaluations on a real internal data set demonstrate the capabilities of Log2NS.

==> figs/bkup_approach.tex <==
%\documentclass[tikz,border=3mm, convert={outfile=compiler.pdf}]{standalone}
%\usepackage{tikz}
\usetikzlibrary{shapes.geometric,positioning,shapes.symbols,shapes.geometric,shadows}
\usetikzlibrary{arrows}
\usepackage{xcolor}
\usetikzlibrary{automata,positioning}
\tikzset{
  multidocument/.style={
    shape=tape,
    draw,
    fill=white,
    tape bend top=none,
    double copy shadow},
  manual input/.style={
    shape=trapezium,
    draw,
    shape border rotate=90,
    trapezium left angle=90,
    trapezium right angle=80}}

\tikzset{
    document/.style={
        shape=tape,
        draw,
        align=center,
        fill=white,
        tape bend top=none,
    }
} 

\begin{document}

\begin{tikzpicture}[>=stealth]

  \node [draw, rounded corners=10pt, minimum width=14cm, minimum height=5cm] at (0,0) (A) {};
  
  \node [draw, rounded corners=10pt, minimum width=6.5cm, minimum height=3cm] at (-3.5,0.5) (B) {};
  \node [draw=white, above = of B, yshift=-1.5cm]  (B3) {\textbf{Machine Learning}};
  \node [draw, fill=gray!20, above = of B, minimum width=3cm, minimum height=1cm] (B1) {Traffic logs};
  \node [draw, minimum width=2.75cm, minimum height=1cm] at (-5,1) (C) {Entity embeddings};
    \node [draw, minimum width=3.15cm, minimum height=1cm] at (-5,-0.25) (D) {Flow vectors};
    \node [draw, minimum width=2.75cm, minimum height=1cm] at (-1.85,1) (E) {Clustering};
    \node [draw, minimum width=2.75cm, minimum height=1cm] at (-1.85,-0.25) (F) {Outlier detection}; 
  
 
  \node [draw, rounded corners=10pt, minimum width=6cm, minimum height=3cm] at (3.5,0.5) (G) {};
  \node [draw=white, above = of G, yshift=-1.5cm]  (B3) {\textbf{Formal}};
   \node [draw, fill=gray!20, above = of G, minimum width=3cm, minimum height=1cm] (G1) {Firewall configs};
  
  
  \node [draw, minimum width=2.5cm, minimum height=1cm] at (4.75,1) (H) {Formal model};
    \node [draw, minimum width=2.5cm, minimum height=1cm] at (4.75,-0.25) (I) {SMT solver};
    \node [draw, minimum width=2.5cm, minimum height=1cm] at (2,1) (J) {Config parser};
    \node [draw, minimum width=2.5cm, minimum height=1cm] at (2,-0.25) (K) {Rule hierarchy}; 
    
    \node [draw, rounded corners=2pt, fill=gray!20, minimum width=12cm, minimum height=0.5cm] at (0,-1.75) (L) {Query Engine}; 
    
    
    \node [multidocument, fill=gray!20, minimum width=2cm, minimum height=1cm]  at  (2,-3.75) (M)         {Results};
    \node [document, fill=gray!20, minimum width=2cm, minimum height=1cm]  at  (-2,-3.75)  (N)        {Queries};
    
    \node [draw=white, fill=gray!10,minimum width=6cm, minimum height=1cm, text width=5cm] at (-4,-5.5) (O1) {\textbf{query}\textbf{(}\textit{srcIP=”10.10.10.1”, \\
      \hspace{3em}destIP=”218.8.104.58”,\\
      \hspace{3em}protocol=[“http”]\textbf{)}}};
    
     \node [draw=white, fill=gray!10,minimum width=7cm, minimum height=1cm, text width=7cm] at (4,-5.5) (P1) {\textbf{result}\textbf{(}\textit{Action=DENY, \\
       \hspace{3.2em}Rule=”Block\_Untrust”,...\textbf{)}}};\textbf{}
    
    \node [draw=white, fill=gray!10,minimum width=6cm, minimum height=1cm, text width=5cm] at (-4,-7.5) (O) {\textbf{query}\textbf{(}\textit{srcIP=NOT(”10.10.10.*”), \\
      \hspace{3em}destIP=”218.8.104.58”,\\
      \hspace{3em}protocol=NOT("udp")\textbf{)}}};
    
     \node [draw=white, fill=gray!10,minimum width=7cm, minimum height=1cm, text width=7cm] at (4,-7.5) (P) {\textbf{result}\textbf{(}\textit{Action=ALLOW, Rule="SC1",\\ 
     \hspace{3em} srcIP=”10.10.45.1” \\
\hspace{3em} destIP=”218.8.104.58”\\
\hspace{3em} protocol=”tcp”, ...\textbf{)}}};\textbf{}
    \node[draw=white]  at  (0,2.75) (B2){\textbf{Log2NS}};

    \node[draw=gray!20, fill=gray!20]  at  (-3.5,-1.85) (B2){};
    \node[draw=gray!20, fill=gray!20]  at  (3.5,-1.85) (G2){};

    \draw [->] (B1) -- (B);  
    \draw [->] (G1) -- (G);  
     \node[draw=white]  at  (0,-3.75) (L2){};
    \draw[implies-implies,double equal sign distance] (B) -- (G);
    \draw[implies-implies,double equal sign distance] (B) -- (B2);
    \draw[implies-implies,double equal sign distance] (G) -- (G2);
    \draw[implies-implies,double equal sign distance] (L) -- (L2);


\end{tikzpicture}
\end{document}

==> figs/intro_chart2.tex <==
%\documentclass[tikz,border=3mm, convert={outfile=compiler.png}]{standalone}
%\usepackage{tikz}
\usetikzlibrary{shapes.geometric,positioning}
%\usepackage{xcolor}
\tikzstyle{every node}=[font=\scriptsize]
%\begin{document}
\begin{center}
\begin{tikzpicture}
\node [draw, fill=gray!20, minimum width=2cm, minimum height=1cm] at (-0.75,0) (A) {Real world};
\node [left=of A, xshift=-0.5cm] (B) {Inputs};
\node [right=of A, xshift=0.5cm] (C) {Outputs};
\node [above=of A, yshift=-0.5cm] (D) {(Model)};
\node [below=of A,yshift=0.5cm] (E) {logs=(inputs, outputs)};

\draw [->] (B) -- (A);
\draw [->] (A) -- (C);
\draw [->,rounded corners=5pt] (B) |- (D);
\draw [->,rounded corners=5pt] (D) -| (C);
\draw [->,rounded corners=5pt] (C) |- (E);
\draw [->,rounded corners=5pt] (E) -| (B);
 %\draw[post,rounded corners=5pt] (D)-|(C);   
\end{tikzpicture}
\end{center}

%\end{document}
